Practical Light Clients for Committee-Based Blockchains

Light clients are gaining increasing attention in the literature since they obviate the need for users to set up dedicated blockchain full nodes. While the literature features a number of light client instantiations, most light client protocols optimize for long offline phases and implicitly assume that the block headers to be verified are signed by highly dynamic validators. In this paper, we show that (i) most light clients are rarely offline for more than a week, and (ii) validators are unlikely to drastically change in most permissioned blockchains and in a number of permissionless blockchains, such as Cosmos and Polkadot. Motivated by these findings, we propose a novel practical system that optimizes for such realistic assumptions and achieves minimal communication and computational costs for light clients when compared to existing protocols. By means of a prototype implementation of our solution, we show that our protocol achieves a reduction by up to $90$ and $40000\times$ (respectively) in end-to-end latency and up to $1000$ and $10000\times$ (respectively) smaller proof size when compared to two state-of-the-art light client instantiations from the literature.

==> arxiv/macros.tex <==
%! TeX root = main.tex

% Math shortcuts that also appear outside math environments can be \def'ed with / for consistent spacing

%------------------------- general

\renewcommand\NN{\mathbb{N}}
\renewcommand\ZZ{\mathbb{Z}}
\renewcommand\FF{\mathbb{F}}
\renewcommand\GG{\mathbb{G}}
\renewcommand\Pr{\mathrm{Pr}}
\renewcommand\concat{\,||\,}
\newcommand\tran{^T}
\newcommand\negl{\mathrm{negl}}

% checkmark and x
\newcommand\cmark{\ding{51}}
\newcommand\xmark{\ding{55}}
\newcommand\rising{\ding{218}}

% empty, filled and half filled circle
\newcommand*{\emptyCircle}{\begin{tikzpicture}[scale=0.11]%
    \draw (0,0) circle (1);
    \end{tikzpicture}}
\newcommand*{\halfCircle}{\begin{tikzpicture}[scale=0.11]%
    \draw (0,0) circle (1);
    \fill (0,0) -- (90:1) arc (90:90-50*3.6:1) -- cycle;
    \end{tikzpicture}}
\newcommand*{\fullCircle}{\begin{tikzpicture}[scale=0.11]%
    \draw (0,0) circle (1);
    \fill (0,0) -- (90:1) arc (90:90-100*3.6:1) -- cycle;
    \end{tikzpicture}}

% spacing after logical and
\newcommand\Land{\land\,}

\newcommand{\bigPr}[2]{%
    \Pr\left[\begin{array}{l}#1\end{array}
    \middle\vert\ 
    \begin{array}{l}#2\end{array}\right]
}

% big probabilities and sets with line break for two column layout
\newcommand{\biggPr}[2]{%
    &\Pr\bigg[\begin{array}{l}#1\end{array}\\
    &\qquad\bigg|\ \begin{array}{l}#2\end{array}\bigg]
}
\newcommand{\BiggPr}[2]{%
    &\Pr\Bigg[\begin{array}{l}#1\end{array}\\
    &\qquad\Bigg|\ \begin{array}{l}#2\end{array}\Bigg]
}
\newcommand{\biggSet}[2]{%
    &\bigg\{\begin{array}{l}#1\end{array}\\
    &\qquad:\ \begin{array}{l}#2\end{array}\bigg\}
}

% \renewcommand\vec[1]{\mathbf{#1}}
% \newcommand\mat[1]{\mathbf{#1}}
\newcommand\schlange[1]{\tilde{#1}}
\newcommand{\idx}[1]{[#1]}
\newcommand{\up}[1]{^{(#1)}}
\newcommand{\down}[1]{_{#1}}

% font for algorithms etc
\newcommand\specialfont[1]{\textsf{#1}}



%------------------------- specific

\newcommand{\subheading}[1]{\vspace{0.5 em}\noindent \textbf{#1}}
\newcommand{\subheadingNoVspace}[1]{\noindent \textbf{#1}}
\newcommand{\sysname}{Awesomeness\xspace}

\newcommand{\missingBlocks}{m}
\newcommand{\m}{\missingBlocks}
\newcommand{\committeeSize}{n}
\newcommand{\startHeight}{\specialfont{h1}}
\newcommand{\heightOld}{\startHeight}
\newcommand\startEpoch{\specialfont{e1}}
\newcommand{\currentEpoch}{\specialfont{e2}}
\newcommand{\heightNew}{\specialfont{h2}}
\newcommand{\currentHeight}{\heightNew}
\newcommand{\quorumSize}{t}
\newcommand{\quorum}{\mathcal{Q}}
\newcommand{\epochLength}{E}

\newcommand{\gtwo}{\hat{g}}
\newcommand{\groupHash}{H}
\newcommand{\step}[1]{\textcircled{#1}}
\newcommand{\apk}{\specialfont{apk}}
\newcommand{\ssk}{\specialfont{ssk}}
\newcommand{\sumKey}{\ssk}
\newcommand{\qsk}{\ssk}
\newcommand{\bitVal}{b}
\newcommand{\bitVec}{\vec{\bitVal}}
\def\NextKeys/{\specialfont{NextK}}
\newcommand{\Nextkeys}{\specialfont{NextK}}
\newcommand{\Hdr}{\specialfont{Hdr}}
\newcommand{\newestHeader}{\Hdr}
% \def\newestHeader/{\Hdr}
\newcommand{\bp}{j}
\newcommand{\breakPoint}{\bp}
\newcommand{\qkeys}{\specialfont{QKeys}}
\newcommand{\keys}[1]{\ensuremath{keys(#1)}\xspace}
\newcommand{\fieldHash}{f}

\newcommand{\KeyGen}{\specialfont{KeyGen}}
% \def\KeyGen/{\specialfont{KeyGen}}
\newcommand{\Sign}{\specialfont{Sign}}
% \def\Sign/{\specialfont{Sign}}
\newcommand{\Verify}{\specialfont{Verify}}
% \def\Verify/{\specialfont{Verify}}
\newcommand{\Aggregate}{\specialfont{Aggregate}}
% \def\Aggregate/{\specialfont{Aggregate}}
\newcommand{\sk}{\specialfont{sk}}
\newcommand{\pk}{\specialfont{pk}}
\newcommand{\PK}{\specialfont{PK}}
\newcommand{\SK}{\specialfont{SK}}
\newcommand{\sig}{s}
\newcommand{\Sig}{S}

\newcommand{\toSign}{x}
\newcommand{\Value}{\toSign}
\renewcommand{\Vector}{\vec{\Value}}
\newcommand{\evalSig}{\Sig}
\newcommand{\functionOutput}{X}
\newcommand{\sumValue}{\functionOutput}
\newcommand{\sumVector}{\vec{\sumValue}}

\def\VerifyAggregate/{\specialfont{Verify}}
\def\Agg/{\Aggregate/}
\def\VerifyAgg/{\VerifyAggregate/}
\def\PoP/{\specialfont{PoP}}
\def\VerifyPoP/{\specialfont{VerifyPoP}}
\def\Eval/{\Aggregate/}
\newcommand{\asBits}[1]{\langle #1 \rangle}
\newcommand{\otherValue}{y}
\newcommand{\thirdValue}{v}
\newcommand{\oneVector}{1^\missingBlocks}
\newcommand{\zeroVector}{0^\missingBlocks}

\newcommand{\setup}{\specialfont{Init}}
\newcommand{\Update}{\specialfont{LC.Update}}
\newcommand{\VerifyState}{\specialfont{LC.Verify}}
\newcommand{\Query}{\specialfont{Query}}
\newcommand{\VerifyResponse}{\specialfont{VerifyResponse}}
%\newcommand{\Submit}{\specialfont{Submit}}
\newcommand{\corresponds}{\specialfont{LCstate}}

\newcommand{\lcState}{d}
\newcommand{\lcStateOld}{\lcState\up{\heightOld}}
\newcommand{\sInit}{\lcState\up{0}}
\newcommand{\sOld}{\lcStateOld}
\newcommand{\sNew}{\lcState\up{\heightNew}}
\newcommand{\validatorsAdv}{\validators_{\mathcal{A}}}
\newcommand{\validatorsAdvCurrent}{\validators_{\mathcal{A}}\up{h}}
\newcommand{\validatorsHonest}{\validators_H}
\newcommand{\validatorsHonestCurrent}{\validators_H\up{h}}
\newcommand{\validatorsCurrent}{\validators\up{\heightOld}}
\newcommand{\validatorsNew}{\validators\up{\heightNew}}
\newcommand{\validatorsThreshold}{f}
\newcommand{\FNClient}{\mathcal{F}}
\newcommand{\FullNode}{\ensuremath{F}}
\newcommand{\BCstateOld}{\BCstate\up{\heightOld}}
\newcommand{\BCstateNew}{\BCstate\up{\heightNew}}
\newcommand{\validators}{\mathcal{V}}
\newcommand{\NbrVal}{\committeeSize}
\newcommand{\BClength}{\heightNew}
\newcommand{\BCstate}{\mathcal{C}}
\newcommand{\advA}{\mathcal{A}}
\newcommand{\advB}{\mathcal{B}}

\newcommand{\User}{u}
\newcommand{\NbrUser}{|U|}
\newcommand{\NbrFN}{c}
\newcommand{\client}{C}
\newcommand{\clients}{\mathcal{C}}
\newcommand{\honestNodes}{\mathcal{N}_H}
\newcommand{\advNodes}{\mathcal{N}_\mathcal{A}}
\newcommand{\nodes}{\mathcal{N}}



% the following are not needed anymore?
% \def\Queries/{\specialfont{Queries}}
% \def\Updates/{\specialfont{Updates}}
% \def\WorldState/{\specialfont{WorldState}}
% \def\PrevHash/{\specialfont{PrevHash}}
% \def\Hash/{\specialfont{Hash}}
% \def\PrevBlock/{\PrevHash/}
% \def\Height/{\specialfont{Height}}
% \def\Epoch/{\specialfont{epoch}}

% \newcommand\com{\mathrm{com}}
% \newcommand\comtilde{\schlange{\com}}
% \def\pp/{\specialfont{pp}}
% \def\Setup/{\specialfont{Setup}}
% \def\Commit/{\specialfont{Commit}}
% \def\Open/{\specialfont{Open}}
% \def\prg/{\specialfont{PRG}}
% \def\prng/{\specialfont{PRG}}

% \newcommand{\prev}{\specialfont{prev}}
% \newcommand{\lab}{i}
% \newcommand{\labelSet}{L}
% \newcommand{\linComb}{w}
% \newcommand{\vectorDim}{d}
% \newcommand{\ped}{\mathrm{Ped}}
% \def\lhsped/{LHS$_\ped$}
% \def\nizk/{\specialfont{NIZK}}
% \def\prover/{\specialfont{P}}
% \def\verifier/{\specialfont{V}}
